Optimizing Pre-Training Data Mixtures with Mixtures of Data Expert Models

We propose a method to optimize language model pre-training data mixtures through efficient approximation of the cross-entropy loss corresponding to each candidate mixture via a Mixture of Data Experts (MDE). We use this approximation as a source of additional features in a regression model, trained from observations of model loss for a small number of mixtures. Experiments with Transformer decoder-only language models in the range of 70M to 1B parameters on the SlimPajama dataset show that our method achieves significantly better performance than approaches that train regression models using only the mixture rates as input features. Combining this improved optimization method with an objective that takes into account cross-entropy on end task data leads to superior performance on few-shot downstream evaluations. We also provide theoretical insights on why aggregation of data expert predictions can provide good approximations to model losses for data mixtures.

==> merged.tex <==

\begin{figure*}[ht!] % or other placement options
\centering
\begin{minipage}[b]{0.60\textwidth} % Adjust width as needed
\centering
\scalebox{.65}{
\begin{tabular}{lcccc}
\toprule
 & MSE \textsc{SP} ($\downarrow$) & $\rho$ \textsc{SP} ($\uparrow$) & MSE ET+SP ($\downarrow$) & $\rho$ ET+SP ($\uparrow$)\\
\midrule
Emp. mean & 0.01151 & N/A & 0.01250 & N/A  \\
\textsc{Linear} & 0.01637 & 0.23426 & 0.00655 & 0.64618 \\
MTGP & 0.00460 & 0.85829 & 0.00231 & 0.89911 \\
\textsc{BiMix}{\tiny{~\cite{bimix}}} & 0.00327 & 0.86051 & N/A  & N/A  \\
DML{\tiny{~\cite{dml}}} & 0.00296 & 0.91991 & 0.00116 & 0.89188 \\
GBM{\tiny{\textsc{RegMix}~\cite{regmix}}} & 0.00242 & 0.92256 & 0.00431 & 0.81442 \\
\midrule
MDE {\tiny{(ours)}} & 0.02809 & 0.91222 & 0.00391 & 0.88571 \\
GBM+MDE {\tiny{(ours)}} & 0.00140 & 0.94963 & 0.00089 & \textbf{0.95462} \\
\textsc{Linear}+MDE {\tiny{(ours)}} & \textbf{0.00050} & 0.97555 & \textbf{0.00048} & 0.95274 \\
MTGP+MDE {\tiny{(ours)}} & 0.00053 & \textbf{0.98383} & 0.00116 & 0.93469 \\
\bottomrule
\end{tabular}
}
%\end{center}
\captionsetup{type=table}
%\captionsetup{name=Table}
\caption{Mean squared error (MSE) and Spearman's rank correlation ($\rho$) on prediction of averaged loss over SlimPajama domains only (\textsc{SP}) and all (\textsc{ET+SP}) validation domains, using different regressors from prior work, and ones proposed in this work.   Regressors are fitted using 25 train mixtures (except MDE that uses only 7 train mixtures), and evaluated with 48 held-out mixtures. MDE features bring large improvements across regressors.}
\label{tab:regressors_sxs}
\end{minipage} % \hfill % Adds horizontal space between minipages
\hfill
% \begin{minipage}[b][][b]{0.31\textwidth}
\begin{minipage}[b]{0.31\textwidth}
\centering
       
 
 \scalebox{.6}{

  \begin{tikzpicture}
    \begin{axis}[
      ylabel={Mean Squared Error (log scale)},
      ymode=log,
      symbolic x coords={ArXiv,Book,C4,CommonCrawl,Github,StackExchange,Wikipedia},
      xtick=data,
      ymin=0.0001,
      ymax=0.2,
      grid=major,
      legend style={at={(0.5,-0.35)}, anchor=north, legend columns=2, draw=none}, % Modified to 2 columns
      x tick label style={rotate=35, anchor=east},
      mark options={solid},
    %   width=0.95\textwidth, % Make the plot wider
    %   height=0.6\textwidth, % Adjust the height to keep aspect ratio
    ]

      % emp. mean
      \addplot[dashed, mark=diamond, color=purple, thick] coordinates {
        (ArXiv,0.03258848761214498) 
        (Book,0.033901799466678983) 
        (C4,0.028237080166221618) 
        (CommonCrawl,0.028170427516745984) 
        (Github,0.04799648997394152) 
        (StackExchange,0.04444072752490156) 
        (Wikipedia,0.16998068744909084)
      };
      \addlegendentry{Emp. Mean}

      % mde
      \addplot[dashed, mark=o, color=green!70!black, thick] coordinates { % Darker green
        (ArXiv,0.12569990165231987) 
        (Book,0.012200067712023305) 
        (C4,0.004183705236557251) 
        (CommonCrawl,0.0038020182635709896) 
        (Github,0.09553608975123355) 
        (StackExchange,0.048190113535861154) 
        (Wikipedia,0.08576905332796389)
      };
      \addlegendentry{MDE (ours)}

      % dml
      \addplot[dashed, mark=triangle*, color=red, thick] coordinates {
        (ArXiv,0.0037785496210790935) 
        (Book,0.0032396400943874803) 
        (C4,0.0022037963338795985) 
        (CommonCrawl,0.0014545846122193365) 
        (Github,0.006231348171967968) 
        (StackExchange,0.01163995357956378) 
        (Wikipedia,0.027135803524510626)
      };
      \addlegendentry{DML}

      % mtgp_mde
      \addplot[dashed, mark=square*, color=blue, thick] coordinates {
        (ArXiv,0.005638437945592803) 
        (Book,0.001197677572446236) 
        (C4,0.0006021703300710033) 
        (CommonCrawl,0.0009188736749797932) 
        (Github,0.0025156553673455454) 
        (StackExchange,0.002369188450940196) 
        (Wikipedia,0.0026375685939519487)
      };
      \addlegendentry{MTGP-\textsc{mde-sp} (ours)}

      % bimix
      \addplot[dashed, mark=star, color=orange, thick] coordinates {
        (ArXiv,0.0014483220708567256) 
        (Book,0.010711812127249159) 
        (C4,0.01641659212707495) 
        (CommonCrawl,0.01133554534292917) 
        (Github,0.010100280035751018) 
        (StackExchange,0.00934835484835737) 
        (Wikipedia,0.0076224179394367726)
      };
      \addlegendentry{BIMIX}

    \end{axis}
  \end{tikzpicture}
  }
  \caption{Per-domain mean loss squared error for SlimPajama validation domains.}
  \label{fig:280M_to_280M_train_only_loss_error_per_domain_sxs}
  \end{minipage}
  
\end{figure*}






% -----


% \begin{figure*}[ht!] % or other placement options
% \centering
% \begin{minipage}[b]{0.66\textwidth} % Adjust width as needed
% \centering
% \scalebox{.65}{
% \begin{tabular}{lcccc}
% \toprule
%  & MSE \textsc{SP} ($\downarrow$) & $\rho$ \textsc{SP} ($\uparrow$) & MSE ET+SP ($\downarrow$) & $\rho$ ET+SP ($\uparrow$)\\
% \midrule
% Emp. mean & 0.01151 & N/A & 0.01250 & N/A  \\
% \textsc{Linear} & 0.01637 & 0.23426 & 0.00655 & 0.64618 \\
% MTGP & 0.00460 & 0.85829 & 0.00231 & 0.89911 \\
% \textsc{BiMix}{\tiny{~\cite{bimix}}} & 0.00327 & 0.86051 & N/A  & N/A  \\
% DML{\tiny{~\cite{dml}}} & 0.00296 & 0.91991 & 0.00116 & 0.89188 \\
% GBM{\tiny{\textsc{RegMix}~\cite{regmix}}} & 0.00242 & 0.92256 & 0.00431 & 0.81442 \\
% \midrule
% MDE {\tiny{(ours)}} & 0.02809 & 0.91222 & 0.00391 & 0.88571 \\
% GBM+MDE {\tiny{(ours)}} & 0.00140 & 0.94963 & 0.00089 & \textbf{0.95462} \\
% \textsc{Linear}+MDE {\tiny{(ours)}} & \textbf{0.00050} & 0.97555 & \textbf{0.00048} & 0.95274 \\
% MTGP+MDE {\tiny{(ours)}} & 0.00053 & \textbf{0.98383} & 0.00116 & 0.93469 \\
% \bottomrule
% \end{tabular}
% }
% %\end{center}
% %\captionsetup{type=table}
% \captionsetup{name=Table}
% \caption{Mean squared error (MSE) and Spearman's rank correlation ($\rho$) on prediction of averaged loss over SlimPajama domains only (\textsc{SP}) and all (\textsc{ET+SP}) validation domains, using different regressors from prior work, and ones proposed in this work.   Regressors are fitted using 25 train mixtures (except MDE that uses only 7 train mixtures), and evaluated with 48 held-out mixtures. MDE features bring large improvements across regressors.}
% \label{tab:regressors_sxs}
% \end{minipage} % \hfill % Adds horizontal space between minipages
% \hfill
% \begin{minipage}[b][][b]{0.31\textwidth}
% \centering
       
 
%  \scalebox{.6}{

%   \begin{tikzpicture}
%     \begin{axis}[
%       ylabel={Mean Squared Error (log scale)},
%       ymode=log,
%       symbolic x coords={ArXiv,Book,C4,CommonCrawl,Github,StackExchange,Wikipedia},
%       xtick=data,
%       ymin=0.0001,
%       ymax=0.2,
%       grid=major,
%       legend style={at={(0.5,-0.35)}, anchor=north, legend columns=2, draw=none}, % Modified to 2 columns
%       x tick label style={rotate=35, anchor=east},
%       mark options={solid},
%     %   width=0.95\textwidth, % Make the plot wider
%     %   height=0.6\textwidth, % Adjust the height to keep aspect ratio
%     ]

%       % emp. mean
%       \addplot[dashed, mark=diamond, color=purple, thick] coordinates {
%         (ArXiv,0.03258848761214498) 
%         (Book,0.033901799466678983) 
%         (C4,0.028237080166221618) 
%         (CommonCrawl,0.028170427516745984) 
%         (Github,0.04799648997394152) 
%         (StackExchange,0.04444072752490156) 
%         (Wikipedia,0.16998068744909084)
%       };
%       \addlegendentry{Emp. Mean}

%       % mde
%       \addplot[dashed, mark=o, color=green!70!black, thick] coordinates { % Darker green
%         (ArXiv,0.12569990165231987) 
%         (Book,0.012200067712023305) 
%         (C4,0.004183705236557251) 
%         (CommonCrawl,0.0038020182635709896) 
%         (Github,0.09553608975123355) 
%         (StackExchange,0.048190113535861154) 
%         (Wikipedia,0.08576905332796389)
%       };
%       \addlegendentry{MDE (ours)}

%       % dml
%       \addplot[dashed, mark=triangle*, color=red, thick] coordinates {
%         (ArXiv,0.0037785496210790935) 
%         (Book,0.0032396400943874803) 
%         (C4,0.0022037963338795985) 
%         (CommonCrawl,0.0014545846122193365) 
%         (Github,0.006231348171967968) 
%         (StackExchange,0.01163995357956378) 
%         (Wikipedia,0.027135803524510626)
%       };
%       \addlegendentry{DML}

%       % mtgp_mde
%       \addplot[dashed, mark=square*, color=blue, thick] coordinates {
%         (ArXiv,0.005638437945592803) 
%         (Book,0.001197677572446236) 
%         (C4,0.0006021703300710033) 
%         (CommonCrawl,0.0009188736749797932) 
%         (Github,0.0025156553673455454) 
%         (StackExchange,0.002369188450940196) 
%         (Wikipedia,0.0026375685939519487)
%       };
%       \addlegendentry{MTGP-\textsc{mde-sp} (ours)}

%       % bimix
%       \addplot[dashed, mark=star, color=orange, thick] coordinates {
%         (ArXiv,0.0014483220708567256) 
%         (Book,0.010711812127249159) 
%         (C4,0.01641659212707495) 
%         (CommonCrawl,0.01133554534292917) 
%         (Github,0.010100280035751018) 
%         (StackExchange,0.00934835484835737) 
%         (Wikipedia,0.0076224179394367726)
%       };
%       \addlegendentry{BIMIX}

%     \end{axis}
%   \end{tikzpicture}
%   }
%   \caption{Per-domain mean loss squared error for SlimPajama validation domains.}
%   \label{fig:280M_to_280M_train_only_loss_error_per_domain_sxs}
%   \end{minipage}
  
% \end{figure*}





==> merged_downstream.tex <==
\begin{figure*}[ht!]
\centering
\begin{minipage}{0.62\textwidth}


  \centering
  \begin{small}
  \begin{sc}
  \scalebox{0.6}{
  \begin{tabular}{@{\hspace{4pt}}l@{\hspace{4pt}}l|c@{\hspace{10pt}}c@{\hspace{8pt}}c@{\hspace{4pt}}c@{\hspace{4pt}}c|c@{\hspace{4pt}}c@{\hspace{4pt}}c@{\hspace{4pt}}c@{\hspace{4pt}}c|c}
  \toprule
  & \multirow{2}{*}{Model} & \multicolumn{5}{c|}{Generation Tasks} & \multicolumn{5}{c|}{Ranking Tasks} & \multirow{2}{*}{Average ($\uparrow$)} \\
    &  & WQ & NQ & \scriptsize{SQuAD} & \scriptsize{TriviaQA} & \scriptsize{LAMBADA} & COPA & PiQA & WiC & \scriptsize{WinoGrande} & \scriptsize{HellaSwag} & \\
  \midrule
    & Uniform & $4.4$  &  $2.4$  &  $35.8$  &  $10.9$  &  ${21.9}$  &  $70.0$  &  $67.9$  &  $49.1$  &  $54.2$  &  $42.3$  &  $35.9$ \\
    & SlimPajama & $\mathbf{6.9}$  &  $\mathbf{3.9}$  &  $37.0$  &  ${15.7}$  &  $18.9$  &  $71.3$  &  $67.2$  &  $49.5$  &  $54.7$  &  $45.3$  &  $37.0$ \\
    & DoGE (124M) & $5.2$  &  $2.3$  &  $33.5$  &  $10.0$  &  $19.9$  &  $70.0$  &  $68.4$  &  $48.1$  &  $54.0$  &  $43.1$  &  $35.4$ \\
    & DoReMi (124M) & $5.1$  &  $2.8$  &  $37.1$  &  $13.6$  &  $21.7$  &  $71.7$  &  $66.4$  &  $48.8$  &  $54.5$  &  $42.3$  &  $36.4$ \\
    \multirow{-5}{*}{\rotatebox[origin=c]{90}{Baselines}}
    & DML & $4.1$  &  $1.9$  &  $34.4$  &  $~~9.1$  &  $15.5$  &  $71.7$  &  $68.1$  &  $\mathbf{50.9}$  &  $54.0$  &  $42.9$  &  $35.3$ \\
  \midrule
    & \textsc{MTGP-mde-sp} & $4.0$  &  $2.4$  &  $34.2$  &  $9.4$  &  $19.6$  &  $68.7$  &  $67.6$  &  $50.4$  &  $52.8$  &  $43.0$  &  $35.2$ \\
    \multirow{-2}{*}{\rotatebox[origin=c]{90}{\scriptsize{Ours}}}
   % & MTGP-MDE-Task & $6.2$  &  $3.3$  &  $\mathbf{39.1}$  &  $14.7$  &  $21.4$  &  $\mathbf{73.7}$  &  $\mathbf{69.7}$  &  $48.7$  &  $\mathbf{57.1}$  &  $\mathbf{46.7}$  &  $\mathbf{38.0}$ \\
 & \textsc{Linear-mde-et} & $6.4$ & $3.5$ & $34.7$ & $\mathbf{17.6}$ & $22.1$ & $\mathbf{75.3}$ & $69.3$ & $49.3$ &  $\mathbf{55.7}$ & $47.6$ & $38.2$ \\
 & \textsc{Linear-mde-all} & $6.1$ & $3.1$ & $\mathbf{37.2}$ & $14.7$ & $\mathbf{24.1}$ & $73.3$ & $\mathbf{70.4}$ & $50.4$ &  $\mathbf{55.7}$ & $\mathbf{47.7}$ & $\mathbf{38.3}$ \\
  \bottomrule
  \end{tabular}
  }
  \end{sc}
  \end{small}
  \caption{Downstream model performance on $5$ prediction tasks and $5$ ranking tasks. Results are averaged across $0$-shot, $1$-shot, and $5$-shot performances.  For generation tasks, we report exact match (EM) accuracies (\%), and for ranking tasks, we report accuracies (\%).  All models are 1B parameter models trained for 200K steps.}
  \label{tab:downstream-results-main-sxs}

\end{minipage} \hfill
\hfill


\begin{minipage}{0.36\textwidth}

\scalebox{0.4}{

\begin{tikzpicture}
    \begin{axis}[
        xlabel={Number of training steps},
        xlabel style={font=\large},
        ylabel={Average downstream accuracy},
        ylabel style={yshift=-12pt, font=\large},
        legend pos=south east,
        ymin=31.0, ymax=39.0,
        xmin=3,xmax=9,
        legend style={at={(1,0)}, anchor=south east},
        ymajorgrids=true,
        grid style=dashed,
        width=12cm,
        height=8cm,
        %xmode=log,
        xtick={3,4,5,6,7, 8, 9}, % Positions for the x-ticks
        xticklabels={50K, 74K, 100K, 126K,150K,174K,200K}, % Custom x-tick labels
        legend style={font=\footnotesize}, % Make legend text smaller
    ]

        \addplot[color=MidnightBlue, line width=1pt, dashed, mark options=solid] coordinates { (3, 32.4) (4, 33.7) (5, 34.0) (6, 35.2) (7, 35.5) (8, 36.0) (9, 35.9)};
        \addlegendentry{Uniform}

        \addplot[color=brown, mark=o, line width=1pt, dashed, mark options=solid] coordinates { (3, 33.7) (4, 34.0) (5, 35.6) (6, 35.5) (7, 35.9) (8, 36.3) (9, 37.0) };
        \addlegendentry{SlimPajama}

        \addplot[color=black, mark=star, line width=1pt, densely dotted, mark options=solid] coordinates { (3, 32.9) (4, 33.6) (5, 34.9) (6, 35.3) (7, 36.2) (8, 35.9) (9, 36.4)};
        \addlegendentry{DoReMi}

        \addplot[color=BrickRed, mark=|, line width=1pt, densely dotted, mark options=solid] coordinates { (3, 32.9) (4, 33.7) (5, 34.0) (6, 34.6) (7, 35.3) (8, 35.3) (9, 35.4) };
        \addlegendentry{DoGE}

        \addplot[color=PineGreen, mark=*, line width=1pt] coordinates { (3, 35.7) (4, 36.8) (5, 36.8) (6, 37.0) (7, 37.6) (8, 37.9) (9, 38.3)};
        \addlegendentry{Linear+\textsc{mde-all}}

        \addplot[color=Plum, mark=diamond*, line width=1pt] coordinates {(3, 35.0) (4, 35.8) (5, 37.2) (6, 37.3) (7, 37.1) (8, 37.6) (9, 38.2)};
        \addlegendentry{Linear+\textsc{mde-et}}

        \addplot[color=VioletRed, mark=oplus, line width=1pt] coordinates { (3, 33.1) (4, 33.5) (5, 34.4) (6, 34.2) (7, 35.0) (8, 34.5) (9, 35.2)};
        \addlegendentry{MTGP+\textsc{mde+sp}}

        \draw [decorate,decoration={brace,amplitude=5pt},yshift=0pt,xshift=250pt]
      (7,25) -- (7,32) node [midway,left,xshift=-5pt] {Prior work};

        \draw [decorate,decoration={brace,amplitude=5pt},yshift=0pt,xshift=250pt]
      (7,5) -- (7,18) node [midway,left,xshift=-5pt] {Ours};
        %\node at (1.2,22) {Ours};

    \end{axis}
\end{tikzpicture}
}
\caption{Downstream task accuracy (average over 0-shot,1-shot, and 5-shot formulations over a suite of generation and ranking tasks) for 1B models optimized through our methods using MDE versus prior work.}
\label{fig:downstream-sxs}
\end{minipage}

\end{figure*}

